libmpk: Software Abstraction for Intel Memory Protection Keys

Intel memory protection keys (MPK) is a new hardware feature to support thread-local permission control on groups of pages without requiring modification of page tables. Unfortunately, its current hardware implementation and software supports suffer from security, scalability, and semantic-gap problems: (1) MPK is vulnerable to protection-key-use-after-free and protection-key corruption; (2) MPK does not scale due to hardware limitations; and (3) MPK is not perfectly compatible with mprotect() because it does not support permission synchronization across threads. In this paper, we propose libmpk, a software abstraction for MPK. libmpk virtualizes protection keys to eliminate the protection-key-use-after-free and protection-key corruption problems while supporting a tremendous number of memory page groups. libmpk also prevents unauthorized writes to its metadata and supports inter-thread key synchronization. We apply libmpk to three real-world applications: OpenSSL, JavaScript JIT compiler, and Memcached for memory protection and isolation. An evaluation shows that libmpk introduces negligible performance overhead (<1%) compared with insecure versions, and improves their performance by 8.1x over secure equivalents using mprotect(). The source code of libmpk will be publicly available and maintained as an open source project.

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> background.tex <==
\section{Background}
\label{s:background}

\XXX{we don't need background.}

% put them in relwk.
% \XXX{page table, \mprotect, extended page table}
% \XXX{domain access control}


\SL{focus on conventional memory access control mechanisms via mprotect, page
  table, TLB, and extended page tables to explain their limitations (mostly
  about their inefficiency and a lack of per-thread control), to eventually come
  up with MPK.}




==> bench12.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4608.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1005,384){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(1005,681){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(1005,978){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(1005,1275){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(1005,1572){\makebox(0,0)[r]{\strut{}$80000$}}%
      \csname LTb\endcsname%%
      \put(1005,1868){\makebox(0,0)[r]{\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(1005,2165){\makebox(0,0)[r]{\strut{}$120000$}}%
      \csname LTb\endcsname%%
      \put(1005,2462){\makebox(0,0)[r]{\strut{}$140000$}}%
      \csname LTb\endcsname%%
      \put(1005,2759){\makebox(0,0)[r]{\strut{}$160000$}}%
      \csname LTb\endcsname%%
      \put(1077,264){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(1448,264){\makebox(0,0){\strut{}$5000$}}%
      \csname LTb\endcsname%%
      \put(1819,264){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(2190,264){\makebox(0,0){\strut{}$15000$}}%
      \csname LTb\endcsname%%
      \put(2562,264){\makebox(0,0){\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(2933,264){\makebox(0,0){\strut{}$25000$}}%
      \csname LTb\endcsname%%
      \put(3304,264){\makebox(0,0){\strut{}$30000$}}%
      \csname LTb\endcsname%%
      \put(3675,264){\makebox(0,0){\strut{}$35000$}}%
      \csname LTb\endcsname%%
      \put(4046,264){\makebox(0,0){\strut{}$40000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(453,1571){\rotatebox{-270}{\makebox(0,0){\strut{}Average Time (cycles)}}}%
      \put(2561,84){\makebox(0,0){\strut{}Number of Loops}}%
      \csname LTb\endcsname%%
      \put(2798,2558){\makebox(0,0)[r]{\strut{}w/ WRPKRU}}%
      \csname LTb\endcsname%%
      \put(2798,2453){\makebox(0,0)[r]{\strut{}w/ WRPKRU (another core)}}%
      \csname LTb\endcsname%%
      \put(2798,2348){\makebox(0,0)[r]{\strut{}w/ CPUID}}%
      \csname LTb\endcsname%%
      \put(2798,2243){\makebox(0,0)[r]{\strut{}w/o WRPKRU}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/bench12}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> bench3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4608.00,2304.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(372,507){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(372,925){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(372,1344){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(372,1762){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(372,2180){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(444,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$0$}}}%
      \csname LTb\endcsname%%
      \put(877,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$5000$}}}%
      \csname LTb\endcsname%%
      \put(1311,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$10000$}}}%
      \csname LTb\endcsname%%
      \put(1744,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$15000$}}}%
      \csname LTb\endcsname%%
      \put(2178,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$20000$}}}%
      \csname LTb\endcsname%%
      \put(2611,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$25000$}}}%
      \csname LTb\endcsname%%
      \put(3044,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$30000$}}}%
      \csname LTb\endcsname%%
      \put(3478,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$35000$}}}%
      \csname LTb\endcsname%%
      \put(3911,435){\rotatebox{30}{\makebox(0,0)[r]{\strut{}$40000$}}}%
      \put(3983,507){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3983,842){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \put(3983,1176){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \put(3983,1511){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \put(3983,1845){\makebox(0,0)[l]{\strut{}$0.8$}}%
      \put(3983,2180){\makebox(0,0)[l]{\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1343){\rotatebox{-270}{\makebox(0,0){\strut{}ms (sparse)}}}%
      \put(4415,1343){\rotatebox{-270}{\makebox(0,0){\strut{}ms (contiguous)}}}%
      \put(2105,87){\makebox(0,0){\strut{}Number of Pages}}%
      \csname LTb\endcsname%%
      \put(1935,2018){\makebox(0,0)[r]{\strut{}mprotect(sparse)}}%
      \csname LTb\endcsname%%
      \put(1935,1862){\makebox(0,0)[r]{\strut{}mprotect(contiguous)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/bench3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> bench4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4608.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1056,384){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1056,645){\makebox(0,0)[r]{\strut{}$5\times10^{6}$}}%
      \csname LTb\endcsname%
      \put(1056,906){\makebox(0,0)[r]{\strut{}$1\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,1168){\makebox(0,0)[r]{\strut{}$1.5\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,1429){\makebox(0,0)[r]{\strut{}$2\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,1690){\makebox(0,0)[r]{\strut{}$2.5\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,1951){\makebox(0,0)[r]{\strut{}$3\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,2213){\makebox(0,0)[r]{\strut{}$3.5\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,2474){\makebox(0,0)[r]{\strut{}$4\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1056,2735){\makebox(0,0)[r]{\strut{}$4.5\times10^{7}$}}%
      \csname LTb\endcsname%
      \put(1128,264){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1495,264){\makebox(0,0){\strut{}$5000$}}%
      \csname LTb\endcsname%
      \put(1863,264){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%
      \put(2230,264){\makebox(0,0){\strut{}$15000$}}%
      \csname LTb\endcsname%
      \put(2598,264){\makebox(0,0){\strut{}$20000$}}%
      \csname LTb\endcsname%
      \put(2965,264){\makebox(0,0){\strut{}$25000$}}%
      \csname LTb\endcsname%
      \put(3332,264){\makebox(0,0){\strut{}$30000$}}%
      \csname LTb\endcsname%
      \put(3700,264){\makebox(0,0){\strut{}$35000$}}%
      \csname LTb\endcsname%
      \put(4067,264){\makebox(0,0){\strut{}$40000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(420,1559){\rotatebox{-270}{\makebox(0,0){\strut{}Average Time (cycles)}}}%
      \put(2597,84){\makebox(0,0){\strut{}Number of Pages}}%
      \csname LTb\endcsname%
      \put(453,269){\makebox(0,0)[r]{\strut{}pkey\_mprotect}}%
      \csname LTb\endcsname%
      \put(453,40){\makebox(0,0)[r]{\strut{}mprotect}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/bench4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chakra-2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8640.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(588,883){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(588,1089){\makebox(0,0)[r]{\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(588,1296){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(588,1502){\makebox(0,0)[r]{\strut{}$30000$}}%
      \csname LTb\endcsname%%
      \put(588,1708){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(588,1914){\makebox(0,0)[r]{\strut{}$50000$}}%
      \csname LTb\endcsname%%
      \put(588,2121){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(588,2327){\makebox(0,0)[r]{\strut{}$70000$}}%
      \csname LTb\endcsname%%
      \put(1069,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Richards}}}%
      \csname LTb\endcsname%%
      \put(1477,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}DeltaBlue}}}%
      \csname LTb\endcsname%%
      \put(1886,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Crypto}}}%
      \csname LTb\endcsname%%
      \put(2294,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RayTrace}}}%
      \csname LTb\endcsname%%
      \put(2703,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}EarleyBoyer}}}%
      \csname LTb\endcsname%%
      \put(3111,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RegExp}}}%
      \csname LTb\endcsname%%
      \put(3520,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Splay}}}%
      \csname LTb\endcsname%%
      \put(3929,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}SplayLatency}}}%
      \csname LTb\endcsname%%
      \put(4337,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}NavierStokes}}}%
      \csname LTb\endcsname%%
      \put(4746,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}PdfJS}}}%
      \csname LTb\endcsname%%
      \put(5154,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Mandreel}}}%
      \csname LTb\endcsname%%
      \put(5563,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}MandreelLatency}}}%
      \csname LTb\endcsname%%
      \put(5972,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Gameboy}}}%
      \csname LTb\endcsname%%
      \put(6380,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}CodeLoad}}}%
      \csname LTb\endcsname%%
      \put(6789,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Box2D}}}%
      \csname LTb\endcsname%%
      \put(7197,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}zlib}}}%
      \csname LTb\endcsname%%
      \put(7606,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Typescript}}}%
      \csname LTb\endcsname%%
      \put(8014,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Total}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1605){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
      \csname LTb\endcsname%%
      \put(1847,2171){\makebox(0,0)[r]{\strut{}Original}}%
      \csname LTb\endcsname%%
      \put(1847,2066){\makebox(0,0)[r]{\strut{}One key per page}}%
      \csname LTb\endcsname%%
      \put(1847,1961){\makebox(0,0)[r]{\strut{}One key per process}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/chakra-2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> chakra.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8640.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(588,883){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(588,1089){\makebox(0,0)[r]{\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(588,1296){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(588,1502){\makebox(0,0)[r]{\strut{}$30000$}}%
      \csname LTb\endcsname%%
      \put(588,1708){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(588,1914){\makebox(0,0)[r]{\strut{}$50000$}}%
      \csname LTb\endcsname%%
      \put(588,2121){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(588,2327){\makebox(0,0)[r]{\strut{}$70000$}}%
      \csname LTb\endcsname%%
      \put(1069,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Richards}}}%
      \csname LTb\endcsname%%
      \put(1477,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}DeltaBlue}}}%
      \csname LTb\endcsname%%
      \put(1886,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Crypto}}}%
      \csname LTb\endcsname%%
      \put(2294,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RayTrace}}}%
      \csname LTb\endcsname%%
      \put(2703,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}EarleyBoyer}}}%
      \csname LTb\endcsname%%
      \put(3111,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RegExp}}}%
      \csname LTb\endcsname%%
      \put(3520,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Splay}}}%
      \csname LTb\endcsname%%
      \put(3929,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}SplayLatency}}}%
      \csname LTb\endcsname%%
      \put(4337,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}NavierStokes}}}%
      \csname LTb\endcsname%%
      \put(4746,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}PdfJS}}}%
      \csname LTb\endcsname%%
      \put(5154,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Mandreel}}}%
      \csname LTb\endcsname%%
      \put(5563,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}MandreelLatency}}}%
      \csname LTb\endcsname%%
      \put(5972,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Gameboy}}}%
      \csname LTb\endcsname%%
      \put(6380,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}CodeLoad}}}%
      \csname LTb\endcsname%%
      \put(6789,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Box2D}}}%
      \csname LTb\endcsname%%
      \put(7197,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}zlib}}}%
      \csname LTb\endcsname%%
      \put(7606,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Typescript}}}%
      \csname LTb\endcsname%%
      \put(8014,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Total}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1605){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
      \csname LTb\endcsname%%
      \put(1847,2171){\makebox(0,0)[r]{\strut{}Original}}%
      \csname LTb\endcsname%%
      \put(1847,2066){\makebox(0,0)[r]{\strut{}One key per page}}%
      \csname LTb\endcsname%%
      \put(1847,1961){\makebox(0,0)[r]{\strut{}One key per process}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/chakra}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> exec-only.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{void}\PY{o}{*} \PY{n+nf}{make\PYZus{}XnR}\PY{p}{(}\PY{k+kt}{size\PYZus{}t} \PY{n}{len}\PY{p}{,} \PY{k+kt}{char} \PY{o}{*}\PY{n}{pie}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k+kt}{void}\PY{o}{*} \PY{n}{addr} \PY{o}{=} \PY{n}{mmap}\PY{p}{(}\PY{n+nb}{NULL}\PY{p}{,} \PY{n}{PAGE\PYZus{}ALIGN}\PY{p}{(}\PY{n}{len}\PY{p}{)}\PY{p}{,} \PY{n}{PROT\PYZus{}WRITE}\PY{p}{,}
                    \PY{n}{MAP\PYZus{}PRIVATE} \PY{o}{|} \PY{n}{MAP\PYZus{}ANONYMOUS}\PY{p}{,} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{,} \PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}

  \PY{c+c1}{// write code to addr}
  \PY{n}{memcpy}\PY{p}{(}\PY{n}{addr}\PY{p}{,} \PY{n}{pie}\PY{p}{,} \PY{n}{len}\PY{p}{)}\PY{p}{;}

  \PY{c+c1}{// page permission: r\PYZhy{}x}
  \PY{c+c1}{// pkey permission: no access (a key is allocated by kernel)}
  \PY{n}{mprotect}\PY{p}{(}\PY{n}{addr}\PY{p}{,} \PY{n}{len}\PY{p}{,} \PY{n}{PROT\PYZus{}EXEC}\PY{p}{)}\PY{p}{;}

  \PY{k}{return} \PY{n}{addr}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> firefox.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(144,1306){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(144,1446){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(144,1586){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(144,1727){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(144,1867){\makebox(0,0)[r]{\strut{}$80000$}}%
      \csname LTb\endcsname%%
      \put(144,2007){\makebox(0,0)[r]{\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-408,1656){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
      \put(2267,2127){\makebox(0,0){\strut{}(a) SpiderMonkey}}%
      \csname LTb\endcsname%%
      \put(4112,2106){\makebox(0,0)[r]{\strut{}mprotect()}}%
      \csname LTb\endcsname%%
      \put(4112,1989){\makebox(0,0)[r]{\strut{}One key per page}}%
      \csname LTb\endcsname%%
      \put(4112,1872){\makebox(0,0)[r]{\strut{}One key per process}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(144,280){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(144,456){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(144,631){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(144,807){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(144,982){\makebox(0,0)[r]{\strut{}$80000$}}%
      \csname LTb\endcsname%%
      \put(432,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Richards}}}%
      \csname LTb\endcsname%%
      \put(648,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}DeltaBlue}}}%
      \csname LTb\endcsname%%
      \put(864,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Crypto}}}%
      \csname LTb\endcsname%%
      \put(1080,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}RayTrace}}}%
      \csname LTb\endcsname%%
      \put(1296,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}EarleyBoyer}}}%
      \csname LTb\endcsname%%
      \put(1512,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}RegExp}}}%
      \csname LTb\endcsname%%
      \put(1728,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Splay}}}%
      \csname LTb\endcsname%%
      \put(1944,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}SplayLatency}}}%
      \csname LTb\endcsname%%
      \put(2160,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}NavierStokes}}}%
      \csname LTb\endcsname%%
      \put(2375,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}PdfJS}}}%
      \csname LTb\endcsname%%
      \put(2591,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Mandreel}}}%
      \csname LTb\endcsname%%
      \put(2807,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}MandreelLatency}}}%
      \csname LTb\endcsname%%
      \put(3023,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Gameboy}}}%
      \csname LTb\endcsname%%
      \put(3239,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}CodeLoad}}}%
      \csname LTb\endcsname%%
      \put(3455,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Box2D}}}%
      \csname LTb\endcsname%%
      \put(3671,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}zlib}}}%
      \csname LTb\endcsname%%
      \put(3887,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Typescript}}}%
      \csname LTb\endcsname%%
      \put(4103,208){\rotatebox{30}{\makebox(0,0)[r]{\strut{}Total}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-336,631){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
      \put(2267,1102){\makebox(0,0){\strut{}(b) ChakraCore}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/firefox}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> impl.tex <==
\section{Implementation}
\label{s:impl}


==> improve.tex <==
\section{Improving Previous Systems}
\label{s:improve}

\XXX{apply MPK to previous security proposals}

\XXX{Execute-only memory}

XOM~\cite{lie:xom00}
XnR~\cite{backes:xnr15}
Redactor~\cite{crane:redactor15}
NEAR~\cite{werner:near16}
Norax~\cite{chen:norax17}

\XXX{JIT}

SDCG~\cite{song:sdcg15}

\XXX{per-thread permission}

Arbiter~\cite{wang:arbiter15}
Shreds~\cite{chen:shreds16}
SMV~\cite{hsu:smv16}

\XXX{STM}

STM~\cite{abadi:stm09}

\XXX{CPI, vtable, ... integrity}

CPI~\cite{kuznetsov:cpi14}
VTint~\cite{zhang:vtint15}


==> lib.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}init}\PY{p}{(}\PY{k+kt}{bool} \PY{n}{cache}\PY{p}{,} \PY{k+kt}{int} \PY{n}{cache\PYZus{}threshold}\PY{p}{,} \PY{k+kt}{bool} \PY{n}{synch}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}mmap}\PY{p}{(}\PY{k+kt}{void}\PY{o}{*}\PY{o}{*} \PY{n}{addr}\PY{p}{,} \PY{k+kt}{void}\PY{o}{*} \PY{n}{addr2}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{length}\PY{p}{,} \PY{k+kt}{int} \PY{n}{prot}\PY{p}{,} 
             \PY{k+kt}{int} \PY{n}{flags}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}mprotect}\PY{p}{(}\PY{k+kt}{int} \PY{n}{id}\PY{p}{,} \PY{k+kt}{int} \PY{n}{prot}\PY{p}{,} \PY{k+kt}{int} \PY{n}{pkey}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}destroy}\PY{p}{(}\PY{k+kt}{int} \PY{n}{id}\PY{p}{,} \PY{k+kt}{int} \PY{n}{pkey}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}begin}\PY{p}{(}\PY{k+kt}{int} \PY{n}{id}\PY{p}{,} \PY{k+kt}{int} \PY{n}{prot}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{mpt\PYZus{}end}\PY{p}{(}\PY{k+kt}{int} \PY{n}{id}\PY{p}{)}\PY{p}{;}
\PY{c+c1}{// int mpt\PYZus{}malloc(void** addr, unsigned long nbytes);}
\PY{c+c1}{// int mpt\PYZus{}free(void* addr);}
\end{Verbatim}


==> mc.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{enum} \PY{n}{store\PYZus{}item\PYZus{}type} \PY{n+nf}{do\PYZus{}store\PYZus{}item}\PY{p}{(}\PY{n}{item} \PY{o}{*}\PY{n}{it}\PY{p}{,} \PY{k+kt}{int} \PY{n}{comm}\PY{p}{,} \PY{n}{conn} \PY{o}{*}\PY{n}{c}\PY{p}{,} 
                                   \PY{k}{const} \PY{k+kt}{uint32\PYZus{}t} \PY{n}{hv}\PY{p}{)} 
\PY{p}{\PYZob{}}
\PY{o}{+} \PY{n}{mpk\PYZus{}begin}\PY{p}{(}\PY{l+m+mi}{2}\PY{p}{,} \PY{n}{PROT\PYZus{}WRITE}\PY{p}{)}\PY{p}{;}
  \PY{k}{volatile} \PY{k}{const} \PY{k+kt}{char} \PY{o}{*}\PY{n}{key} \PY{o}{=} \PY{n}{ITEM\PYZus{}key}\PY{p}{(}\PY{n}{it}\PY{p}{)}\PY{p}{;}
  \PY{k}{volatile} \PY{k}{const} \PY{k+kt}{size\PYZus{}t} \PY{n}{nkey} \PY{o}{=} \PY{n}{it}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{nkey}\PY{p}{;}
\PY{o}{+} \PY{n}{mpk\PYZus{}end}\PY{p}{(}\PY{l+m+mi}{2}\PY{p}{)}\PY{p}{;}
  \PY{n}{item} \PY{o}{*}\PY{n}{old\PYZus{}it} \PY{o}{=} \PY{n}{do\PYZus{}item\PYZus{}get}\PY{p}{(}\PY{p}{(}\PY{k}{const} \PY{k+kt}{char}\PY{o}{*}\PY{p}{)}\PY{n}{key}\PY{p}{,} \PY{n}{nkey}\PY{p}{,} \PY{n}{hv}\PY{p}{)}\PY{p}{;} 
  \PY{k}{enum} \PY{n}{store\PYZus{}item\PYZus{}type} \PY{n}{stored} \PY{o}{=} \PY{n}{NOT\PYZus{}STORED}\PY{p}{;}

  \PY{n}{item} \PY{o}{*}\PY{n}{new\PYZus{}it} \PY{o}{=} \PY{n+nb}{NULL}\PY{p}{;}
  \PY{k+kt}{int} \PY{n}{flags}\PY{p}{;}

  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> microbench.js.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{// N.js}

\PY{k+kd}{function} \PY{n+nx}{f\PYZus{}1}\PY{p}{(}\PY{n+nx}{a}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o}{=} \PY{l+m+mi}{1}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{=} \PY{l+m+mi}{1}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{2}\PY{p}{]} \PY{o}{=} \PY{l+m+mi}{1}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]} \PY{o}{=}  \PY{l+m+mi}{1}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kd}{var} \PY{n+nx}{a\PYZus{}X} \PY{o}{=} \PY{k}{new} \PY{n+nb}{Array}\PY{p}{(}\PY{l+m+mi}{4}\PY{p}{)}\PY{p}{;}
\PY{k}{for} \PY{p}{(}\PY{k+kd}{let} \PY{n+nx}{i} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;} \PY{n+nx}{i} \PY{o}{\PYZlt{}} \PY{l+m+mi}{100000}\PY{p}{;} \PY{n+nx}{i}\PY{o}{++}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n+nx}{f\PYZus{}X}\PY{p}{(}\PY{n+nx}{a\PYZus{}X}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{p}{...}

\PY{k+kd}{function} \PY{n+nx}{f\PYZus{}N}\PY{p}{(}\PY{n+nx}{a}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o}{=} \PY{n+nx}{N}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{=} \PY{n+nx}{N}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{2}\PY{p}{]} \PY{o}{=} \PY{n+nx}{N}\PY{p}{;} \PY{n+nx}{a}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]} \PY{o}{=}  \PY{n+nx}{N}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kd}{var} \PY{n+nx}{a\PYZus{}N} \PY{o}{=} \PY{k}{new} \PY{n+nb}{Array}\PY{p}{(}\PY{l+m+mi}{4}\PY{p}{)}\PY{p}{;}
\PY{k}{for} \PY{p}{(}\PY{k+kd}{let} \PY{n+nx}{i} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;} \PY{n+nx}{i} \PY{o}{\PYZlt{}} \PY{l+m+mi}{100000}\PY{p}{;} \PY{n+nx}{i}\PY{o}{++}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n+nx}{f\PYZus{}N}\PY{p}{(}\PY{n+nx}{a\PYZus{}N}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> no-hide.tex <==
\begin{tabular}{lr}
  \toprule
  % Instruction/operation & Cycles (4\KB)& Cycles (1\B) \\
    \textbf{Instruction/operation} & \textbf{Elapsed cycles} \\
  \midrule
    %SFI (and) & 1524.31 & < 0.4 \\
    %MPX (single \bndcu) & 603.64 & < 0.2 \\
    %MPX (both \bndcu and \bndcl) & 3012.25 & 0.74 \\
     MPK (simulated) & 63.35 \\
  %    MPK (simulated) & 63.35 & 63.35 \\
      MPK (real hardware) & 48.34 \\
  %    MPK (real hardware) & 48.34 & 48.34 \\
    %AES encrpytion and decryption\dag & 50028.60 & 50028.60\\
%  \midrule
%  \dag domain-based isolation\\
  \bottomrule
\end{tabular}


==> novel.tex <==
\section{Novel Applications}
\label{s:novel}

\XXX{novel security or system applications}

\XXX{exclusive write, per-instruction or per-basic-block memory protection}

\XXX{thread sanitizer}


==> openssl.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{static} \PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}rsa\PYZus{}decrypt}\PY{p}{(}\PY{n}{EVP\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{ctx}\PY{p}{,}
                            \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{out}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{o}{*}\PY{n}{outlen}\PY{p}{,}
                            \PY{k}{const} \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{in}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{inlen}\PY{p}{)}
\PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{ret}\PY{p}{;}
    \PY{n}{RSA\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{rctx} \PY{o}{=} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{data}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode} \PY{o}{=}\PY{o}{=} \PY{n}{RSA\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}PADDING}\PY{p}{)} \PY{p}{\PYZob{}}
        \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{setup\PYZus{}tbuf}\PY{p}{(}\PY{n}{rctx}\PY{p}{,} \PY{n}{ctx}\PY{p}{)}\PY{p}{)}
            \PY{k}{return} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                  \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,} \PY{n}{RSA\PYZus{}NO\PYZus{}PADDING}\PY{p}{)}\PY{p}{;}
        \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{)}
            \PY{k}{return} \PY{n}{ret}\PY{p}{;}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}padding\PYZus{}check\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}mgf1}\PY{p}{(}\PY{n}{out}\PY{p}{,} \PY{n}{ret}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                                \PY{n}{ret}\PY{p}{,} \PY{n}{ret}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}label}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}labellen}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{md}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{mgf1md}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}} \PY{k}{else}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{out}\PY{p}{,} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,}
                                  \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0}\PY{p}{)}
        \PY{k}{return} \PY{n}{ret}\PY{p}{;}
    \PY{o}{*}\PY{n}{outlen} \PY{o}{=} \PY{n}{ret}\PY{p}{;}
    \PY{k}{return} \PY{l+m+mi}{1}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> openssl.mpk.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{static} \PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}rsa\PYZus{}decrypt}\PY{p}{(}\PY{n}{EVP\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{ctx}\PY{p}{,}
                            \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{out}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{o}{*}\PY{n}{outlen}\PY{p}{,}
                            \PY{k}{const} \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{in}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{inlen}\PY{p}{)}
\PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{ret}\PY{p}{;}
    \PY{n}{RSA\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{rctx} \PY{o}{=} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{data}\PY{p}{;}
\PY{o}{+}   \PY{n}{mpk\PYZus{}begin}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{,} \PY{n}{PROT\PYZus{}WRITE}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode} \PY{o}{=}\PY{o}{=} \PY{n}{RSA\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}PADDING}\PY{p}{)} \PY{p}{\PYZob{}}
      \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{setup\PYZus{}tbuf}\PY{p}{(}\PY{n}{rctx}\PY{p}{,} \PY{n}{ctx}\PY{p}{)}\PY{p}{)} \PY{p}{\PYZob{}}
\PY{o}{\PYZhy{}}       \PY{k}{return} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
\PY{o}{+}       \PY{n}{ret} \PY{o}{=} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
\PY{o}{+}       \PY{k}{goto} \PY{n}{out}\PY{p}{;}
      \PY{p}{\PYZcb{}}
      \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,} \PY{n}{RSA\PYZus{}NO\PYZus{}PADDING}\PY{p}{)}\PY{p}{;}
      \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{)} 
\PY{o}{\PYZhy{}}       \PY{k}{return} \PY{n}{ret}\PY{p}{;}
\PY{o}{+}       \PY{k}{goto} \PY{n}{out}\PY{p}{;}
      \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}padding\PYZus{}check\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}mgf1}\PY{p}{(}\PY{n}{out}\PY{p}{,} \PY{n}{ret}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                              \PY{n}{ret}\PY{p}{,} \PY{n}{ret}\PY{p}{,}
                                              \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}label}\PY{p}{,}
                                              \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}labellen}\PY{p}{,}
                                              \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{md}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{mgf1md}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}} \PY{k}{else}
      \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{out}\PY{p}{,} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,}
                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0}\PY{p}{)}
\PY{o}{\PYZhy{}}     \PY{k}{return} \PY{n}{ret}\PY{p}{;}
\PY{o}{+}     \PY{k}{goto} \PY{n}{out}\PY{p}{;}

    \PY{o}{*}\PY{n}{outlen} \PY{o}{=} \PY{n}{ret}\PY{p}{;}
\PY{o}{\PYZhy{}}   \PY{k}{return} \PY{l+m+mi}{1}\PY{p}{;}
\PY{o}{+}   \PY{n}{ret} \PY{o}{=} \PY{l+m+mi}{1}\PY{p}{;}
\PY{o}{+}\PY{n+nl}{out}\PY{p}{:}
\PY{o}{+}   \PY{n}{mpk\PYZus{}end}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{;}
\PY{o}{+}   \PY{k}{return} \PY{n}{ret}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> openssl.ori.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{static} \PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}rsa\PYZus{}decrypt}\PY{p}{(}\PY{n}{EVP\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{ctx}\PY{p}{,}
                            \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{out}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{o}{*}\PY{n}{outlen}\PY{p}{,}
                            \PY{k}{const} \PY{k+kt}{unsigned} \PY{k+kt}{char} \PY{o}{*}\PY{n}{in}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{inlen}\PY{p}{)}
\PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{ret}\PY{p}{;}
    \PY{n}{RSA\PYZus{}PKEY\PYZus{}CTX} \PY{o}{*}\PY{n}{rctx} \PY{o}{=} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{data}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode} \PY{o}{=}\PY{o}{=} \PY{n}{RSA\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}PADDING}\PY{p}{)} \PY{p}{\PYZob{}}
        \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{setup\PYZus{}tbuf}\PY{p}{(}\PY{n}{rctx}\PY{p}{,} \PY{n}{ctx}\PY{p}{)}\PY{p}{)}
            \PY{k}{return} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                  \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,} \PY{n}{RSA\PYZus{}NO\PYZus{}PADDING}\PY{p}{)}\PY{p}{;}
        \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{)}
            \PY{k}{return} \PY{n}{ret}\PY{p}{;}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}padding\PYZus{}check\PYZus{}PKCS1\PYZus{}OAEP\PYZus{}mgf1}\PY{p}{(}\PY{n}{out}\PY{p}{,} \PY{n}{ret}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{tbuf}\PY{p}{,}
                                                \PY{n}{ret}\PY{p}{,} \PY{n}{ret}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}label}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{oaep\PYZus{}labellen}\PY{p}{,}
                                                \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{md}\PY{p}{,} \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{mgf1md}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}} \PY{k}{else}
        \PY{n}{ret} \PY{o}{=} \PY{n}{RSA\PYZus{}private\PYZus{}decrypt}\PY{p}{(}\PY{n}{inlen}\PY{p}{,} \PY{n}{in}\PY{p}{,} \PY{n}{out}\PY{p}{,} \PY{n}{ctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pkey}\PY{p}{.}\PY{n}{rsa}\PY{p}{,}
                                  \PY{n}{rctx}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{pad\PYZus{}mode}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{ret} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0}\PY{p}{)}
        \PY{k}{return} \PY{n}{ret}\PY{p}{;}
    \PY{o}{*}\PY{n}{outlen} \PY{o}{=} \PY{n}{ret}\PY{p}{;}
    \PY{k}{return} \PY{l+m+mi}{1}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> overhead-flush.tex <==
\begin{tabular}{lr}
  \toprule
  \textbf{Instructions} & \textbf{Elapsed cycles} \\
  \midrule
  WRPKRU  & 23.1 \\
  WRPKRU with 15 instructions before WRPKRU  & 25.2  \\
  WRPKRU with 15 instructions after WRPKRU & 32.7 \\
  \bottomrule
\end{tabular}


==> overhead-instr.tex <==
\begin{tabular}{lr}
  \toprule
  \textbf{Instruction} & \textbf{Elapsed cycles} \\
  \midrule
  RDPKRU  & 0.53 \\
  WRPKRU  & 23.31  \\
%   WRPKRU after RDPKRU & 24.45  \\
  \midrule
  MOVQ (\rbx to \rdx) & 0.0 \\
  MOVQ (\rdx to \xmm) & 2.09 \\
  \bottomrule
\end{tabular}


==> overhead-syscall.tex <==
\begin{tabular}{lr}
\toprule
  \textbf{System call} & \textbf{Elapsed cycles} \\
\midrule
  mprotect & 1093.99 \\
  pkey\_mprotect & 1104.90 \\
  pkey\_alloc &186.28 \\
  pkey\_free & 137.22 \\
\bottomrule
\end{tabular}


==> pkey-libc-func.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}get} \PY{p}{(}\PY{k+kt}{int} \PY{n}{key}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{key} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0} \PY{o}{|}\PY{o}{|} \PY{n}{key} \PY{o}{\PYZgt{}} \PY{l+m+mi}{15}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n}{\PYZus{}\PYZus{}set\PYZus{}errno} \PY{p}{(}\PY{n}{EINVAL}\PY{p}{)}\PY{p}{;}
      \PY{k}{return} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
  \PY{p}{\PYZcb{}}
  \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{pkru} \PY{o}{=} \PY{n}{pkey\PYZus{}read} \PY{p}{(}\PY{p}{)}\PY{p}{;}
  \PY{k}{return} \PY{p}{(}\PY{n}{pkru} \PY{o}{\PYZgt{}}\PY{o}{\PYZgt{}} \PY{p}{(}\PY{l+m+mi}{2} \PY{o}{*} \PY{n}{key}\PY{p}{)}\PY{p}{)} \PY{o}{\PYZam{}} \PY{l+m+mi}{3}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}set} \PY{p}{(}\PY{k+kt}{int} \PY{n}{key}\PY{p}{,} \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{rights}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{key} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0} \PY{o}{|}\PY{o}{|} \PY{n}{key} \PY{o}{\PYZgt{}} \PY{l+m+mi}{15} \PY{o}{|}\PY{o}{|} \PY{n}{rights} \PY{o}{\PYZgt{}} \PY{l+m+mi}{3}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n}{\PYZus{}\PYZus{}set\PYZus{}errno} \PY{p}{(}\PY{n}{EINVAL}\PY{p}{)}\PY{p}{;}
    \PY{k}{return} \PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{;}
  \PY{p}{\PYZcb{}}
  \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{mask} \PY{o}{=} \PY{l+m+mi}{3} \PY{o}{\PYZlt{}}\PY{o}{\PYZlt{}} \PY{p}{(}\PY{l+m+mi}{2} \PY{o}{*} \PY{n}{key}\PY{p}{)}\PY{p}{;}
  \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{pkru} \PY{o}{=} \PY{n}{pkey\PYZus{}read} \PY{p}{(}\PY{p}{)}\PY{p}{;}
  \PY{n}{pkru} \PY{o}{=} \PY{p}{(}\PY{n}{pkru} \PY{o}{\PYZam{}} \PY{o}{\PYZti{}}\PY{n}{mask}\PY{p}{)} \PY{o}{|} \PY{p}{(}\PY{n}{rights} \PY{o}{\PYZlt{}}\PY{o}{\PYZlt{}} \PY{p}{(}\PY{l+m+mi}{2} \PY{o}{*} \PY{n}{key}\PY{p}{)}\PY{p}{)}\PY{p}{;}
  \PY{n}{pkey\PYZus{}write} \PY{p}{(}\PY{n}{pkru}\PY{p}{)}\PY{p}{;}
  \PY{k}{return} \PY{l+m+mi}{0}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{c+c1}{// System call wrappers for pkey\PYZus{}alloc, pkey\PYZus{}free, pkey\PYZus{}mprotect}
\end{Verbatim}


==> pkey-syscall.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}mprotect}\PY{p}{(}\PY{k+kt}{void} \PY{o}{*}\PY{n}{addr}\PY{p}{,} \PY{k+kt}{size\PYZus{}t} \PY{n}{len}\PY{p}{,} \PY{k+kt}{int} \PY{n}{prot}\PY{p}{,} \PY{k+kt}{int} \PY{n}{pkey}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{c+c1}{// internal}
\PY{p}{\PYZcb{}}

\PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}alloc}\PY{p}{(}\PY{k+kt}{unsigned} \PY{k+kt}{long} \PY{n}{flags}\PY{p}{,} \PY{k+kt}{unsigned} \PY{k+kt}{long} \PY{n}{access\PYZus{}rights}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{c+c1}{// internal}
\PY{p}{\PYZcb{}}

\PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}free}\PY{p}{(}\PY{k+kt}{int} \PY{n}{pkey}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{c+c1}{// internal}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> pkey-wrap.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{// \PYZlt{}arch\PYZhy{}pkey.h\PYZgt{}}
\PY{k}{static} \PY{k+kr}{inline} \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n+nf}{pkey\PYZus{}read} \PY{p}{(}\PY{k+kt}{void}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{result}\PY{p}{;}
  \PY{n}{\PYZus{}\PYZus{}asm\PYZus{}\PYZus{}} \PY{k}{volatile} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{.byte 0x0f, 0x01, 0xee}\PY{l+s}{\PYZdq{}} \PY{c+c1}{// rdpkru}
                    \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{=a}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{n}{result}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{rdx}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{;}
  \PY{k}{return} \PY{n}{result}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k}{static} \PY{k+kr}{inline} \PY{k+kt}{void} \PY{n+nf}{pkey\PYZus{}write} \PY{p}{(}\PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{value}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{\PYZus{}\PYZus{}asm\PYZus{}\PYZus{}} \PY{k}{volatile} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{.byte 0x0f, 0x01, 0xef}\PY{l+s}{\PYZdq{}} \PY{c+c1}{// wrpkru}
                    \PY{o}{:} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{a}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{n}{value}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{d}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> pkru.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{define make\PYZus{}pkru(pkey, rights) (rights \PYZlt{}\PYZlt{} (2 * pkey))}

\PY{k+kt}{void} \PY{n+nf}{wrpkru}\PY{p}{(}\PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{pkru}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{asm} \PY{k}{volatile}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{.byte 0x0f,0x01,0xef}\PY{l+s+se}{\PYZbs{}n}\PY{l+s+se}{\PYZbs{}t}\PY{l+s}{\PYZdq{}}
               \PY{o}{:} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{a}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{n}{pkru}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{d}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kt}{int} \PY{n+nf}{rdpkru}\PY{p}{(}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{register} \PY{k+kt}{int} \PY{n}{eax}\PY{p}{,} \PY{n}{edx}\PY{p}{;}
  \PY{k}{asm} \PY{k}{volatile}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{.byte 0x0f, 0x01, 0xee}\PY{l+s+se}{\PYZbs{}n}\PY{l+s+se}{\PYZbs{}t}\PY{l+s}{\PYZdq{}}
               \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{=a}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{n}{eax}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{=d}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{n}{edx}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{\PYZdq{}} \PY{p}{(}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{)}\PY{p}{;}
  \PY{k}{return} \PY{n}{eax}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> syscall.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4608.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(444,240){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(444,596){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(444,953){\makebox(0,0)[r]{\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(444,1309){\makebox(0,0)[r]{\strut{}$300$}}%
      \csname LTb\endcsname%
      \put(444,1666){\makebox(0,0)[r]{\strut{}$400$}}%
      \csname LTb\endcsname%
      \put(444,2022){\makebox(0,0)[r]{\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(444,2379){\makebox(0,0)[r]{\strut{}$600$}}%
      \csname LTb\endcsname%
      \put(444,2735){\makebox(0,0)[r]{\strut{}$700$}}%
      \csname LTb\endcsname%
      \put(1000,120){\makebox(0,0){\strut{}mprotect}}%
      \csname LTb\endcsname%
      \put(1969,120){\makebox(0,0){\strut{}pkey_mprotect}}%
      \csname LTb\endcsname%
      \put(2938,120){\makebox(0,0){\strut{}pkey_alloc}}%
      \csname LTb\endcsname%
      \put(3907,120){\makebox(0,0){\strut{}pkey_free}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(96,1487){\rotatebox{-270}{\makebox(0,0){\strut{}Cycles}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/syscall}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tbl/tbl-security.tex <==
\begin{tabular}{llll}
\toprule
\textbf{Application} & \textbf{Domain-based isolation} & \textbf{Fast \mprotect} & \textbf{Per-thread isolation} \\
\midrule
OpenSSL & \checkmark & & \checkmark \\
JIT & & \checkmark & \checkmark \\
memcached & \checkmark & & \checkmark \\
\bottomrule
\end{tabular}


==> threat.tex <==



==> v8.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\footnotesize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(588,883){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(588,1076){\makebox(0,0)[r]{\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(588,1268){\makebox(0,0)[r]{\strut{}$20000$}}%
      \csname LTb\endcsname%%
      \put(588,1461){\makebox(0,0)[r]{\strut{}$30000$}}%
      \csname LTb\endcsname%%
      \put(588,1654){\makebox(0,0)[r]{\strut{}$40000$}}%
      \csname LTb\endcsname%%
      \put(588,1846){\makebox(0,0)[r]{\strut{}$50000$}}%
      \csname LTb\endcsname%%
      \put(588,2039){\makebox(0,0)[r]{\strut{}$60000$}}%
      \csname LTb\endcsname%%
      \put(841,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Richards}}}%
      \csname LTb\endcsname%%
      \put(1022,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}DeltaBlue}}}%
      \csname LTb\endcsname%%
      \put(1204,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Crypto}}}%
      \csname LTb\endcsname%%
      \put(1385,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RayTrace}}}%
      \csname LTb\endcsname%%
      \put(1566,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}EarleyBoyer}}}%
      \csname LTb\endcsname%%
      \put(1747,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}RegExp}}}%
      \csname LTb\endcsname%%
      \put(1928,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Splay}}}%
      \csname LTb\endcsname%%
      \put(2110,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}SplayLatency}}}%
      \csname LTb\endcsname%%
      \put(2291,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}NavierStokes}}}%
      \csname LTb\endcsname%%
      \put(2472,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}PdfJS}}}%
      \csname LTb\endcsname%%
      \put(2653,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Mandreel}}}%
      \csname LTb\endcsname%%
      \put(2835,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}MandreelLatency}}}%
      \csname LTb\endcsname%%
      \put(3016,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Gameboy}}}%
      \csname LTb\endcsname%%
      \put(3197,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}CodeLoad}}}%
      \csname LTb\endcsname%%
      \put(3378,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Box2D}}}%
      \csname LTb\endcsname%%
      \put(3559,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}zlib}}}%
      \csname LTb\endcsname%%
      \put(3741,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Typescript}}}%
      \csname LTb\endcsname%%
      \put(3922,811){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Total}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(108,1461){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
      \csname LTb\endcsname%%
      \put(4004,1988){\makebox(0,0)[r]{\strut{}Original}}%
      \csname LTb\endcsname%%
      \put(4004,1848){\makebox(0,0)[r]{\strut{}libmpk}}%
      \csname LTb\endcsname%%
      \put(4004,1708){\makebox(0,0)[r]{\strut{}SDCG}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/v8}}%
    \gplfronttext
  \end{picture}%
\endgroup

